BD-KD: Balancing the Divergences for Online Knowledge Distillation

We address the challenge of producing trustworthy and accurate compact models for edge devices. While Knowledge Distillation (KD) has improved model compression in terms of achieving high accuracy performance, calibration of these compact models has been overlooked. We introduce BD-KD (Balanced Divergence Knowledge Distillation), a framework for logit-based online KD. BD-KD enhances both accuracy and model calibration simultaneously, eliminating the need for post-hoc recalibration techniques, which add computational overhead to the overall training pipeline and degrade performance. Our method encourages student-centered training by adjusting the conventional online distillation loss on both the student and teacher losses, employing sample-wise weighting of forward and reverse Kullback-Leibler divergence. This strategy balances student network confidence and boosts performance. Experiments across CIFAR10, CIFAR100, TinyImageNet, and ImageNet datasets, and various architectures demonstrate improved calibration and accuracy compared to recent online KD methods.

==> TSNE.tex <==
\begin{comment}

\begin{figure}
\begin{minipage}{\linewidth}
    \begin{minipage}{\textwidth}
    \centering
       \includegraphics[width=\linewidth]{Figures/capacity_gap_curves.png}
       \vspace{-0.4cm}
    \captionof{figure}{\textbf{Capacity Gap curve.} Student (ResNet20) distilled different teacher capacity (WRN16-2 to WRN-16-8) on CIFAR100.}
    \label{fig:capacity_gap_curve}
    \end{minipage}
   \begin{minipage}{0.5\linewidth}
    \begin{minipage}{\textwidth}
        \includegraphics[width=\linewidth]{Figures/switch_tsne_100perp.png}
        \centering{(a) SwitOKD \cite{qian2022switchable}}
    \end{minipage}%
    \begin{minipage}{\linewidth}
        \includegraphics[width=\linewidth]{Figures/tsne_ours_sample_weighting_perplexity100.png}
    \centering{(b) BD-KD (ours) }
    \end{minipage}
    \end{minipage}
    \vspace{-0.1cm}
   \captionof{figure}{Visualization results of features on the test images from CIFAR10 with t-SNE \cite{van2008visualizing}. Table\ref{tab:sota_final}}
   \label{fig:tsne}
\end{minipage}
\end{figure}
    
\end{comment}

\begin{figure}
\begin{minipage}{0.5\linewidth}
    \begin{minipage}{\textwidth}
        \includegraphics[width=\linewidth]{Figures/switch_tsne_100perp.png}
        \centering{(a) SwitOKD \cite{qian2022switchable}}
    \end{minipage}%
    \begin{minipage}{\linewidth}
        \includegraphics[width=\linewidth]{Figures/tsne_ours_sample_weighting_perplexity100.png}
    \centering{(b) BD-KD (ours) }
    \end{minipage}
    \end{minipage}
    \vspace{-0.1cm}
   \captionof{figure}{Visualization results of features on the test images from CIFAR10 with t-SNE \cite{van2008visualizing}. Table\ref{tab:sota_final}}
   \label{fig:tsne}
\end{figure}


==> Tables/ablation_type_losses.tex <==
\begin{table}[h]
%\begin{wraptable}{r}{0.5\textwidth}
\caption{Ablation on different KD Losses.}
\label{tab:ablation_losses}
%(CRD \cite{tian2019contrastive}, DKD\cite{zhao2022decoupled} and SHAKE \cite{li2022shake}).}
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lrcc} 
    \toprule
    $S$ KD Loss & $T$ KD Loss &  Student Acc. & Teacher Acc. \\
    \midrule
    \multirow{3}{}{$KL_{forward}$} & $KL_{forward}$
    & 75.63 & 78.05 \\   
     & $KL_{reverse}$
    & 76.12 & 78.84\\
     & $KL_{JSD}$
    & 76.24 & 78.56 \\
    \midrule
    \multirow{3}{}{$KL_{reverse}$} & $KL_{forward}$
    & 75.71 & 78.29 \\
    & $KL_{reverse}$ 
    & 76.2 & 79.09\\
    & $KL_{JSD}$ 
    &76.2 & 78.55\\
    \midrule
    \multirow{3}{}{$KL_{JSD}$ }& $KL_{forward}$ 
    & 76.63 & 78.7\\
     & $KL_{reverse}$
    & \textbf{76.83} & \textbf{79.08}\\
    & $KL_{JSD}$ 
    & 76.19 & 78.64\\
    \midrule
    \midrule
    \multicolumn{2}{}{BDKD (Eq. \ref{eq:student_obj} and Eq. \ref{eq:teacher_obj}) }& AA & BB \\
    \bottomrule
\end{tabular}
}
%\end{wraptable}
\end{table}


==> Tables/hpt_sensitivity_t.tex <==
\begin{table}[h]
%\begin{wraptable}{r}{0.4\textwidth}
\centering
\caption{\textbf{Hyperparameter sensitivity.} Illustrating the effect of varying the temperature value $\tau$ on CIFAR-100. We report both teacher and student accuracies. }
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
        \multicolumn{2}{c}{Networks} & $\tau=1$   & $\tau=2$   & $\tau=3$ & $\tau=4$ \\ \midrule
Student & WRN\_16\_2  & 75.51 & \textbf{76.42} & 76.37 & 76.30 \\
Teacher & WRN\_16\_40 & 78.00 & 78.80 & 79.02  & 78.92 \\ \bottomrule
\end{tabular}
}
\label{tab:temp_ablation2}
\end{table}
%\end{wraptable}
%

==> Tables/hpt_sensitivity_v.tex <==
% \begin{table}[h]
% %\begin{wraptable}{l}{0.4\textwidth}
% \caption{\footnotesize{\textbf{Hyperparameter sensitivity.} Illustrating the effect of varying the hyperparameter $v$ on CIFAR-100 with different network architectures. We report both teacher and student accuracies.}}
% \label{tab:vparam}
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{lllll}
% \toprule
%              & \multicolumn{1}{c}{v=1} & \multicolumn{1}{c}{v=2} & \multicolumn{1}{c}{v=3} & \multicolumn{1}{c}{v=4} \\ \midrule
% VGG8 (S)     & 74.48                  & 74.95                   & \textbf{75.05}                   & 74.80                   \\
% VGG13 (T)    & 76.25                   & 76.43                   & 76.83                   & 76.76                   \\ \midrule
% ResNet20 (S) & 71.90                   &  \textbf{72.04}                  & 71.70                   & 71.72                   \\
% WRN-40-2 (T) & 77.19                   &  77.31                  & 77.58                   & 77.83                    \\ \bottomrule
% \end{tabular}
% }
% \label{tab:temp_ablation1}
% \end{table}
% %\end{wraptable}

%%%%%%%%%%%%%% ONLY ONE LINE 
\begin{table}[h]
%\begin{wraptable}{l}{0.4\textwidth}
\caption{\footnotesize{\textbf{Hyperparameter sensitivity.} Illustrating the effect of varying the hyperparameter $v$ on CIFAR-100. We report both teacher and student accuracies.}}
\label{tab:vparam}
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllll}
\toprule
             & \multicolumn{1}{c}{v=1} & \multicolumn{1}{c}{v=2} & \multicolumn{1}{c}{v=3} & \multicolumn{1}{c}{v=4} \\ \midrule
ResNet20 (S) & 71.90                   &  \textbf{72.04}                  & 71.70                   & 71.72                   \\
WRN-40-2 (T) & 77.19                   &  77.31                  & 77.58                   & 77.83                    \\ \bottomrule
\end{tabular}
}
\label{tab:temp_ablation1}
\end{table}
%\end{wraptable}

==> Tables/new_ablation.tex <==
%\begin{wraptable}{r}{0.4\textwidth}
\begin{table}[h]
%\caption{\footnote{The caption}}
\centering
\caption{Accuracy and ECE of student and teacher models under offline KD.}
\label{tab:new_ablation}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccc}
    \toprule
         KD\tiny{strategy-CIFAR100}&  \multicolumn{2}{c}{Accuracy
T/S}& ECE\\
\midrule
 Vanilla& 75.84& 75.06& 6.45\%\\
 Vanilla + BDKD EQ2& 75.84&  \greenup 75.43& \greendown4.02\%\\
 Vanilla  + JSD& 75.84& 75.34&5.1\%\\
 \midrule
 DML& 78.57& 75.81&3.60 \%\\
 DML +BDKD EQ2& 78.29&  \greenup 75.89 & \greendown 3.20 \%\\
 DML + JSD& 78.35& 75.82&3.51\%\\
 \midrule
 SwitOKD& 75.84& 74.90&4.40 \%\\
 SwitOKD + BDKD EQ2& 77.10&  \greenup 75.93& \greendown 3.21 \%\\
 \midrule
 \midrule
 BDKD (OURS)& 78.44& \textbf{76.26}& \textbf{3.00\%}\\
 \bottomrule
\end{tabular}
}
%\end{wraptable}
\end{table}
% \small{T:WRN40-2; S:WRN-16-2}

==> Tables/performance_accuracy_tables.tex <==
% \begin{table}[h]
% %\begin{wraptable}{r}{3cm}
% \begin{minipage}{0.6\linewidth}
% \caption{ Accuracy (\%) comparison of student network performances with other KD techniques using similar architectures (SA) or different architecture (DA). Gain(KD) and Gain(DML) represent, respectively, the performance improvement over the classical KD and online KD baseline DML. Most Values are taken from \cite{zhao2022decoupled} and \cite{li2022shake}, and values with (*) are from our own implementation.}
% \label{tab:offlinekd}
% %(CRD \cite{tian2019contrastive}, DKD\cite{zhao2022decoupled} and SHAKE \cite{li2022shake}).}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ lcccccc} \toprule
%         &\multicolumn{3}{c}{\textbf{Same Architecture}} &  \multicolumn{3}{c}{\textbf{Different Architecture}} \\\midrule
%         Teacher & WRN-40-2 & R32x4 & VGG13  & VGG13 & R50 & R32x4 \\
%         Student & WRN-16-2 & R8x4  & VGG8   & MV2   & VGG8 & ShV2  \\ \midrule
%         Teacher & 75.61    & 79.42 & 74.64  & 74.64 & 79.34 & 79.42 \\ 
%         Student & 73.26    & 72.50 & 70.36 & 64.60 & 70.36 & 71.82 \\ \midrule
%         Vanilla KD
%         \cite{hinton2015distilling} & 74.92 & 73.33 & 72.98 & 67.37& 73.81 & 74.45 \\ 
%         FitNets
%         \cite{romero2014fitnets}    & 73.58  & 73.50 & 71.02 & 64.14 & 70.69 & 73.54 \\
%         CRD 
%         \cite{tian2019contrastive}      & 75.48 & 75.51 & 73.94 & 69.73 & 74.30 & 75.65 \\
%         DKD 
%         \cite{zhao2022decoupled}      & 76.24 & 76.32 & 74.68 & 69.71 & N/A & 77.07 \\
%         \midrule
%         DML
%         \cite{dml}      & 75.33   & 74.30 & 73.64 & 68.52 & 74.22& 75.71 *\\
%         KDCL
%         \cite{kdcl}     & 74.25    & 74.03 & 71.26 & 65.76  & 73.03 & N/A  \\    %SwitchOKD$\ssymbol{4}$ & 75.95 & bbbbbbbb & ccccccc & ddddddd & eeeeee & ------ \\
%         SHAKE
%         \cite{li2022shake} & 76.62   & 77.35 &74.84  & 70.03& 74.76 & N/A  \\
%         BD-KD (Ours) & 76.47 & 76.67 & \textbf{74.96} & 69.33 & \textbf{74.87} & 76.95 \\
%         Gain (KD) & \textcolor{green}{+ 1.55} &\textcolor{green}{+ 3.34} & \textcolor{green} {+ 1.98} & \textcolor{green}{+ 1.96} & \textcolor{green}{+ 1.06} & \textcolor{green}{+ 2.5}     \\
%         Gain (DML) & \textcolor{green}{+ 1.14} & \textcolor{green}{+ 2.37} & \textcolor{green}{+ 1.32} & \textcolor{green}{+ 0.81} & \textcolor{green}{+ 0.65} & \textcolor{green}{+ 1.24}\\
%         \bottomrule
        
% \end{tabular}
% }
% %\end{wraptable}
% % \end{table}
% \end{minipage}
% %
% \begin{minipage}{0.4\linewidth}
% \begin{minipage}{0.3\linewidth}
% \caption{\footnotesize Top-1 and top-5 accuracy (\%) on the ImageNet validation set. We used ResNet50 to be our teacher network and MobileNetV1 as our student. (*) and (**) values are taken from \cite{li2022shake} and \cite{zhao2022decoupled}. respectively.}
% \label{tab:imagenet2}
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{lcc} \toprule
%                 KD Method & Top-1 & Top-5 \\ \midrule
%                 KD \cite{hinton2015distilling}         & 70.68 &  90.30 \\
%                 CRD \cite{tian2019contrastive}         & 71.40 & 90.42 \\
%                 ReviewKD \cite{chen2021distilling}   & 72.56 &  91.00 \\
%                 DKD \cite{zhao2022decoupled}         & 72.05 & 91.05 \\
%                 AT \cite{zagoruyko2016paying};\cite{mirzadeh2020improved}         & 70.72 &  90.03 \\
%                 RKD \cite{park2019relational}        & 71.32 &  90.62  \\
%                 DML \cite{dml}         & 71.13 &  90.22  \\
%                 SHAKE  \cite{li2022shake}     & 72.66 &  91.35 \\ 
%                 BD-KD (Ours) & \textbf{72.97 } & 90.98 \\
%                 \bottomrule
                
                       
% \end{tabular}}
% %\end{table}    
% \end{minipage}
% \begin{minipage}{0.2\linewidth}
%     %\begin{figure}
%     \centering
%        \includegraphics[width=\linewidth]{Figures/capacity_gap_curves.png}
%     \captionof{figure}{\footnotesize \textbf{Capacity Gap curve.} Student (ResNet20) distilled different teacher capacity (WRN16-2 to WRN-16-8) on CIFAR100.}
%     \label{fig:capacity_gap_curve}
% %\end{figure}
% \end{minipage}
%
% \end{table}    
\begin{figure}[th]
\resizebox{\textwidth}{!}{
%    \begin{minipage}[t]{0.4\textwidth}
    \captionof{table}{Accuracy (\%) comparison of student network performances with other KD techniques using similar architectures (SA) or different architecture (DA). Gain(KD) and Gain(DML) represent, respectively, the performance improvement over the classical KD and online KD baseline DML. Most values are taken from \cite{zhao2022decoupled} and \cite{li2022shake}, and values with (*) are from our own implementation.}
        \label{tab:offlinekd}
        \centering
        %First table (left panel)
        \resizebox{\textwidth}{!}{
        \begin{tabular}{ lcccccc} \toprule
        &\multicolumn{3}{c}{\textbf{Same Architecture}} &  \multicolumn{3}{c}{\textbf{Different Architecture}} \\\midrule
        Teacher & WRN-40-2 & R32x4 & VGG13  & VGG13 & R50 & R32x4 \\
        Student & WRN-16-2 & R8x4  & VGG8   & MV2   & VGG8 & ShV2  \\ \midrule
        Teacher & 75.61    & 79.42 & 74.64  & 74.64 & 79.34 & 79.42 \\ 
        Student & 73.26    & 72.50 & 70.36 & 64.60 & 70.36 & 71.82 \\ \midrule
        Vanilla KD
        \cite{hinton2015distilling} & 74.92 & 73.33 & 72.98 & 67.37& 73.81 & 74.45 \\ 
        FitNets
        \cite{romero2014fitnets}    & 73.58  & 73.50 & 71.02 & 64.14 & 70.69 & 73.54 \\
        CRD 
        \cite{tian2019contrastive}      & 75.48 & 75.51 & 73.94 & 69.73 & 74.30 & 75.65 \\
        DKD 
        \cite{zhao2022decoupled}      & 76.24 & 76.32 & 74.68 & 69.71 & N/A & 77.07 \\
        \midrule
        DML
        \cite{dml}      & 75.33   & 74.30 & 73.64 & 68.52 & 74.22& 75.71 *\\
        KDCL
        \cite{kdcl}     & 74.25    & 74.03 & 71.26 & 65.76  & 73.03 & N/A  \\    %SwitchOKD$\ssymbol{4}$ & 75.95 & bbbbbbbb & ccccccc & ddddddd & eeeeee & ------ \\
        SHAKE
        \cite{li2022shake} & 76.62   & 77.35 &74.84  & 70.03& 74.76 & N/A  \\
        BD-KD (Ours) & 76.47 & 76.67 & \textbf{74.96} & 69.33 & \textbf{74.87} & 76.95 \\
        Gain (KD) & \textcolor{green}{+ 1.55} &\textcolor{green}{+ 3.34} & \textcolor{green} {+ 1.98} & \textcolor{green}{+ 1.96} & \textcolor{green}{+ 1.06} & \textcolor{green}{+ 2.5}     \\
        Gain (DML) & \textcolor{green}{+ 1.14} & \textcolor{green}{+ 2.37} & \textcolor{green}{+ 1.32} & \textcolor{green}{+ 0.81} & \textcolor{green}{+ 0.65} & \textcolor{green}{+ 1.24}\\
        \bottomrule
        
\end{tabular} 
}
%    \end{minipage}
    \hspace{1mm}
%    \begin{minipage}[t]{0.4\textwidth}
    \captionof{table}{Top-1 and top-5 accuracy (\%) on the ImageNet validation set. We used ResNet50 to be our teacher network and MobileNetV1 as our student. 
    % (*) and (**) values are taken from \cite{li2022shake} and \cite{zhao2022decoupled}. respectively.}
    }
\label{tab:imagenet2}
        \centering
        % Second table (right panel, top)
        \resizebox{0.55\textwidth}{9mm}{
        \begin{tabular}{lcc} \toprule
                KD Method & Top-1 & Top-5 \\ \midrule
                KD \cite{hinton2015distilling}         & 70.68 &  90.30 \\
                CRD \cite{tian2019contrastive}         & 71.40 & 90.42 \\
                ReviewKD \cite{chen2021distilling}   & 72.56 &  91.00 \\
                DKD \cite{zhao2022decoupled}         & 72.05 & 91.05 \\
                AT \cite{zagoruyko2016paying};\cite{mirzadeh2020improved}         & 70.72 &  90.03 \\
                RKD \cite{park2019relational}        & 71.32 &  90.62  \\
                DML \cite{dml}         & 71.13 &  90.22  \\
                SHAKE  \cite{li2022shake}     & 72.66 &  91.35 \\ 
                BD-KD (Ours) & \textbf{72.97 } & 90.98 \\
                \bottomrule
              
\end{tabular}
} 
% \end{minipage}
        % Image (right panel, bottom)
        %\vspace{1mm} % adjust the vertical space between the table and image as needed
        \includegraphics[width=0.8\textwidth, height=22mm]{Figures/capacity_gap_curves.png}
    \captionof{figure}{\textbf{Capacity Gap curve.} Student (ResNet20) distilled different teacher capacity (WRN16-2 to WRN-16-8) on CIFAR100.}
    \label{fig:capacity_gap_curve}
%     \end{minipage}
}
\end{figure}

==> algorithms.tex <==
\begin{algorithm}[ht]
\begin{minipage}{0.2\linewidth}
\SetAlgoLined
\footnotesize
    \PyComment{x:input image} \\
    \PyComment{y:ground truth} \\
    \PyComment{model\_s: student model} \\
    \PyComment{model\_t: teacher model} \\
    \PyComment{H\_s, H\_t: entropy student and teacher} \\
    \PyComment{$v$: hyper-parameter related to BD-KD} \\
    \PyComment{alpha\_s,alpha\_t,beta\_s,beta\_t: hyper parameters related to KD} \\
    \PyCode{for (x,y) in Batches:} \\
    \Indp   % start indent
        \PyComment{values of logits} \\
        \PyCode{output\_t = model\_t(x)} \\ 
        \PyCode{output\_s = model\_s(x)} \\ 
        \PyComment{calculate the ce losses} \\
        \PyCode{loss\_ce\_t = beta\_t * ce\_loss(output\_t, y)}\\
        \PyCode{loss\_ce\_s = beta\_s * ce\_loss(output\_s, y)}\\
        \PyComment{calculate the kl loss teacher} \\
        \PyCode{loss\_kl\_t = T*T*alpha\_t * kl\_div\_loss(output\_t, output\_s.detach())}\\
        \PyComment{teacher total loss} \\
        \PyCode{total\_loss\_t= loss\_ce\_t + loss\_kl\_t }\\
        \PyComment{calculate entropy gap} \\
        \PyCode{H\_gap = H\_s - H\_t}\\
        \PyComment{initializing sample weights} \\
        \PyCode{delta\_reverse = 1}\\
        \PyCode{delta\_forward = 1}\\
        \PyCode{if H\_gap $\geq$ 0: }\\
        \Indp
            \PyCode{delta\_reverse = $v$}\\
        \Indm 
        \PyCode{else: }\\
         \Indp
            \PyCode{delta\_forward = $v$}\\
        \Indm 
        \PyComment{calculate the kl loss student} \\
        \PyCode{loss\_kl\_s = T*T*alpha\_s * \\weighted\_kl\_div\_loss(output\_s,output\_t.detach(), delta\_reverse) + \\ weighted\_kl\_div\_loss(output\_t.detach(),output\_s, delta\_forward)}\\
        \PyComment{student total loss} \\
         \PyCode{total\_loss\_s = loss\_ce\_t + loss\_kl\_s}\\
        \PyComment{updates} \\
        \PyCode{total\_loss\_t.backward()}\\
        \PyCode{total\_loss\_s.backward()}\\
    \Indm % end indent, must end with this, 
\caption{PyTorch-style pseudocode for BD-KD}
\label{algo:your-algo}
\end{minipage}
\end{algorithm}
%\end{minipage}


==> capacity_gap.tex <==
\begin{figure}
%\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
       \includegraphics[width=0.4\linewidth]{Figures/capacity_gap_curves.png}
    \captionof{figure}{\footnotesize \textbf{Capacity Gap curve.} Student (ResNet20) distilled from different teacher capacity (WRN16-2 to WRN-16-8) on CIFAR100.}
    \label{fig:capacity_gap_curve}
\end{figure}
%\end{wrapfigure}

==> combine_forward_backward.tex <==
%\begin{figure}[h]
\begin{wrapfigure}{r}{0.4\textwidth}
\scalebox{0.8}{
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=1.3\linewidth]{Figures/ablation_loss_student.png}
    \centering{(a) Student (WRN-16-2) Accuracy }
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=1.3\linewidth]{Figures/ablation_loss_teacher.png}
    \centering{(b) Teacher (WRN-40-2) Accuracy }
    \end{minipage}
}
\caption{\footnotesize \textbf{Ablation study}. Understanding the effect of different combinations of forward, reverse, and symmetric KL divergences for online distillation training. Results back up the motivation behind the design of the objective functions of our proposed method. }
\label{fig:ablation_loss}
%\end{figure}
\end{wrapfigure}

==> entropy_evolution.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\begin{center}
\includegraphics[width=\linewidth]{Figures/final_entropy_gap.png}
\end{center}
\caption{
{\footnotesize \textbf{Entropy Evolution.} 
}}
\label{fig:framework}
%\end{figure}
\end{wrapfigure}

==> tsne_cifar100.tex <==
\begin{figure}[h!]
    \begin{minipage}{0.26\textwidth}
    \includegraphics[width=\textwidth]{tsne_bdkd_res32x4_teacher_perp100.png}
    \centering{(a) }
    \end{minipage}%
    \begin{minipage}{0.26\textwidth}
    \includegraphics[width=\textwidth]{tsne_switch_res32x4_teacher_perp100.png}
    \centering{(b) }
    \end{minipage}
    \caption{\textbf{T-SNE on CIFAR100} }
    \label{fig:}
\end{figure}

\begin{figure}[h!]
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\linewidth]{tsne_bdkd_shufflev2_student_perp100.png}    
    \centering{(c)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\linewidth]{tsne_switch_shufflev2_student_perp100.png}
    \centering{(d)}
    \end{minipage}
    \caption{\textbf{T-SNE on CIFAR100} }
    \label{fig:sup2}
\end{figure}

\begin{figure}[h!]
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\linewidth]{tsne_bdkd_vgg13bn_teacher_perp100.png}
    \centering{(a) }
    \end{minipage}
    \hfill
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\linewidth]{tsne_switch_vgg13bn_teacher_perp100.png}
    \centering{(b) }
    \end{minipage}
    
    \caption{\textbf{T-SNE on CIFAR100} }
    \label{fig:sup2}
\end{figure}
